AlleNoise: large-scale text classification benchmark dataset with real-world label noise

Label noise remains a challenge for training robust classification models. Most methods for mitigating label noise have been benchmarked using primarily datasets with synthetic noise. While the need for datasets with realistic noise distribution has partially been addressed by web-scraped benchmarks such as WebVision and Clothing1M, those benchmarks are restricted to the computer vision domain. With the growing importance of Transformer-based models, it is crucial to establish text classification benchmarks for learning with noisy labels. In this paper, we present AlleNoise, a new curated text classification benchmark dataset with real-world instance-dependent label noise, containing over 500,000 examples across approximately 5,600 classes, complemented with a meaningful, hierarchical taxonomy of categories. The noise distribution comes from actual users of a major e-commerce marketplace, so it realistically reflects the semantics of human mistakes. In addition to the noisy labels, we provide human-verified clean labels, which help to get a deeper insight into the noise distribution, unlike web-scraped datasets typically used in the field. We demonstrate that a representative selection of established methods for learning with noisy labels is inadequate to handle such real-world noise. In addition, we show evidence that these algorithms do not alleviate excessive memorization. As such, with AlleNoise, we set the bar high for the development of label noise methods that can handle real-world label noise in text classification tasks. The code and dataset are available for download at https://github.com/allegro/AlleNoise.

==> figure-allenoise-simple.tex <==

\begin{figure}
    \centering
    \begin{tabular}{|l|lll|l|l|}
\hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Observed \\ category\end{tabular}} & \multicolumn{3}{c|}{Clean examples}              & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Symmetric noise \\ examples\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}AlleNoise \\ examples\end{tabular}} \\ \hline
\begin{tabular}[c]{@{}l@{}} Pendant lamps \end{tabular}                  
& \multicolumn{1}{l|}{\includegraphics[height=0.12\textwidth]{figures-allenoise/lampa1.jpeg}   }
& \multicolumn{1}{l|}{\includegraphics[height=0.12\textwidth]{figures-allenoise/lampa2.jpeg}} 
&  \includegraphics[height=0.12\textwidth]{figures-allenoise/lampa3.jpeg}
& \includegraphics[height=0.12\textwidth]{figures-allenoise/szczoteczka.jpeg}     
& \includegraphics[height=0.12\textwidth]{figures-allenoise/plafon.jpeg}     \\ \hline
& \multicolumn{1}{l|}{} 
& \multicolumn{1}{l|}{} 
&  
& \begin{tabular}[c]{@{}l@{}} Electric \\toothbrushes \end{tabular}                      
& \begin{tabular}[c]{@{}l@{}} Ceiling Domes \end{tabular}                 \\ \hline
\begin{tabular}[c]{@{}l@{}}Winter tires  \end{tabular}             
& \multicolumn{1}{l|}{\includegraphics[height=0.12\textwidth]{figures-allenoise/opona1.jpeg}   }
& \multicolumn{1}{l|}{\includegraphics[height=0.12\textwidth]{figures-allenoise/opona2.jpeg}} 
&  \includegraphics[height=0.12\textwidth]{figures-allenoise/opona3.jpeg}
& \includegraphics[height=0.12\textwidth]{figures-allenoise/jezdzik.jpeg}     
& \includegraphics[height=0.12\textwidth]{figures-allenoise/alleason.jpeg}     \\ \hline
& \multicolumn{1}{l|}{}
& \multicolumn{1}{l|}{} 
& 
& \begin{tabular}[c]{@{}l@{}} Ride Ons \end{tabular}        
& \begin{tabular}[c]{@{}l@{}} All-season \\tires \end{tabular}                     \\ \hline
\end{tabular}
    \caption{Depiction of the difference between symmetric synthetic noise and AlleNoise. Symmetric synthetic noise is unlikely to provide misleading examples. AlleNoise noisy examples are hard to detect even for untrained humans. AlleNoise dataset does not include images. We use images only to provide clear depiction of AlleNoise. 
}
    \label{fig:fig1-allenoise}
\end{figure}

==> figure-allenoise.tex <==

\begin{figure}
    \centering
    \begin{tabular}{|l|lll|l|l|}
\hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Observed \\ category\end{tabular}} & \multicolumn{3}{c|}{Clean examples}              & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Symmetric noise \\ examples\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}AlleNoise \\ examples\end{tabular}} \\ \hline
\begin{tabular}[c]{@{}l@{}}Home and Garden>\\Lighting>Lamps \\
Pendant lamps \end{tabular}                  
& \multicolumn{1}{l|}{\includegraphics[height=0.15\textwidth]{figures-allenoise/lampa1.jpeg}   }
& \multicolumn{1}{l|}{\includegraphics[height=0.15\textwidth]{figures-allenoise/lampa2.jpeg}} 
&  \includegraphics[height=0.15\textwidth]{figures-allenoise/lampa3.jpeg}
& \includegraphics[height=0.15\textwidth]{figures-allenoise/szczoteczka.jpeg}     
& \includegraphics[height=0.15\textwidth]{figures-allenoise/plafon.jpeg}     \\ \hline
& \multicolumn{1}{l|}{} 
& \multicolumn{1}{l|}{} 
&  
& \begin{tabular}[c]{@{}l@{}}
Health>Oral hygiene\\
>Toothbrush>Electric\end{tabular}                      
& \begin{tabular}[c]{@{}l@{}}Home and Garden>\\Lighting>Lamps \\
Ceiling Domes \\and Half Domes \end{tabular}                 \\ \hline
\begin{tabular}[c]{@{}l@{}}Automotive\\>Tires and Rims> \\Tires\\>For passenger cars\\>Winter   \end{tabular}             
& \multicolumn{1}{l|}{\includegraphics[height=0.15\textwidth]{figures-allenoise/opona1.jpeg}   }
& \multicolumn{1}{l|}{\includegraphics[height=0.15\textwidth]{figures-allenoise/opona1.jpeg}} 
&  \includegraphics[height=0.15\textwidth]{figures-allenoise/opona3.jpeg}
& \includegraphics[height=0.15\textwidth]{figures-allenoise/jezdzik.jpeg}     
& \includegraphics[height=0.15\textwidth]{figures-allenoise/alleason.jpeg}     \\ \hline
& \multicolumn{1}{l|}{}
& \multicolumn{1}{l|}{} 
& 
& \begin{tabular}[c]{@{}l@{}}
Kids\\>Bicycles and Vehicles\\>Ride Ons \end{tabular}        
& \begin{tabular}[c]{@{}l@{}}Automotive\\>Tires and Rims\\>Tires\\>For passenger cars\\>All-season \end{tabular}                     \\ \hline
\end{tabular}
    \caption{Graphical depiction of the difference between symmetric synthetic noise and AlleNoise. Symmetric synthetic noise is unlikely to provide misleading examples. AlleNoise noisy examples are hard to detect even for untrained humans. AlleNoise dataset does not include images. We use images only to provide clear depiction of AlleNoise. 
}
    \label{fig:fig1-allenoise}
\end{figure}

==> figures-results/allenoise_clean_correct.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{coral}{RGB}{255,127,80}
\definecolor{crimson}{RGB}{220,20,60}
\definecolor{cyan}{RGB}{0,255,255}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{gold}{RGB}{255,215,0}
\definecolor{limegreen}{RGB}{50,205,50}
\definecolor{purple}{RGB}{128,0,128}
\definecolor{teal}{RGB}{0,128,128}
\definecolor{violet}{RGB}{238,130,238}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Step},
xmin=0, xmax=15000,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Correct clean},
ymin=0.353019753263036, ymax=0.768653433036161,
ytick style={color=black}
]
\path [draw=limegreen, fill=limegreen, opacity=0.1]
(axis cs:1412,0.516706358579787)
--(axis cs:1412,0.511571637136604)
--(axis cs:2825,0.608168747925354)
--(axis cs:4238,0.655827409550625)
--(axis cs:5651,0.682376376513153)
--(axis cs:7064,0.704133083680136)
--(axis cs:8477,0.717115853600781)
--(axis cs:9890,0.725443008306704)
--(axis cs:11303,0.73022085121759)
--(axis cs:12716,0.734196568264675)
--(axis cs:14129,0.736222034246699)
--(axis cs:14129,0.741584782377087)
--(axis cs:14129,0.741584782377087)
--(axis cs:12716,0.740057021586557)
--(axis cs:11303,0.735589885600968)
--(axis cs:9890,0.730473454305077)
--(axis cs:8477,0.71976037099933)
--(axis cs:7064,0.707244702647093)
--(axis cs:5651,0.688989545777282)
--(axis cs:4238,0.659836102516618)
--(axis cs:2825,0.61264411930119)
--(axis cs:1412,0.516706358579787)
--cycle;

\path [draw=crimson, fill=crimson, opacity=0.1]
(axis cs:1412,0.516666485794949)
--(axis cs:1412,0.512660733393575)
--(axis cs:2825,0.605203300050057)
--(axis cs:4238,0.652888956422565)
--(axis cs:5651,0.68032798121834)
--(axis cs:7064,0.699024420955313)
--(axis cs:8477,0.712995111380371)
--(axis cs:9890,0.720622086363078)
--(axis cs:11303,0.728273429808065)
--(axis cs:12716,0.731393740817996)
--(axis cs:14129,0.733665971466334)
--(axis cs:14129,0.740338923373145)
--(axis cs:14129,0.740338923373145)
--(axis cs:12716,0.737757212111341)
--(axis cs:11303,0.734711121954324)
--(axis cs:9890,0.728702692952082)
--(axis cs:8477,0.720442301841838)
--(axis cs:7064,0.707534027821562)
--(axis cs:5651,0.687471585934292)
--(axis cs:4238,0.657638203065)
--(axis cs:2825,0.614301879457861)
--(axis cs:1412,0.516666485794949)
--cycle;

\path [draw=coral, fill=coral, opacity=0.1]
(axis cs:0,0.746544659079669)
--(axis cs:0,0.612055511050345)
--(axis cs:0,0.746544659079669)
--(axis cs:0,0.746544659079669)
--cycle;

\path [draw=gold, fill=gold, opacity=0.1]
(axis cs:1412,0.464680596963592)
--(axis cs:1412,0.371912193252724)
--(axis cs:2825,0.519212035098835)
--(axis cs:4238,0.58328178582123)
--(axis cs:5651,0.61975658153692)
--(axis cs:7064,0.644984159572231)
--(axis cs:8477,0.663624558943898)
--(axis cs:9890,0.678576351942674)
--(axis cs:11303,0.687471245115639)
--(axis cs:12716,0.694906685006449)
--(axis cs:14129,0.699792287543442)
--(axis cs:14129,0.70950873854527)
--(axis cs:14129,0.70950873854527)
--(axis cs:12716,0.705179935798842)
--(axis cs:11303,0.698841141455108)
--(axis cs:9890,0.688754800287398)
--(axis cs:8477,0.675158267505514)
--(axis cs:7064,0.660193414437594)
--(axis cs:5651,0.637925337292791)
--(axis cs:4238,0.608126378499388)
--(axis cs:2825,0.559227410864582)
--(axis cs:1412,0.464680596963592)
--cycle;

\path [draw=purple, fill=purple, opacity=0.1]
(axis cs:1412,0.516591187766823)
--(axis cs:1412,0.511796490387401)
--(axis cs:2825,0.606108962809593)
--(axis cs:4238,0.652209742235681)
--(axis cs:5651,0.682578017170296)
--(axis cs:7064,0.7011706246774)
--(axis cs:8477,0.715524174180528)
--(axis cs:9890,0.720671777615943)
--(axis cs:11303,0.728514897727276)
--(axis cs:12716,0.731893758216434)
--(axis cs:14129,0.734201252072582)
--(axis cs:14129,0.740332358330714)
--(axis cs:14129,0.740332358330714)
--(axis cs:12716,0.738148802968285)
--(axis cs:11303,0.73530267215413)
--(axis cs:9890,0.728363172889974)
--(axis cs:8477,0.719628469994103)
--(axis cs:7064,0.704404308562509)
--(axis cs:5651,0.684564414452461)
--(axis cs:4238,0.657427570404246)
--(axis cs:2825,0.608103867210629)
--(axis cs:1412,0.516591187766823)
--cycle;

\path [draw=blue, fill=blue, opacity=0.1]
(axis cs:1412,0.529997190504234)
--(axis cs:1412,0.520411965683673)
--(axis cs:2825,0.612199984686547)
--(axis cs:4238,0.658882870987768)
--(axis cs:5651,0.683245213260128)
--(axis cs:7064,0.704706291006979)
--(axis cs:8477,0.714162473708663)
--(axis cs:9890,0.722122235715122)
--(axis cs:11303,0.727661413463352)
--(axis cs:12716,0.731010468604768)
--(axis cs:14129,0.732395512815886)
--(axis cs:14129,0.738478977508418)
--(axis cs:14129,0.738478977508418)
--(axis cs:12716,0.736781643889918)
--(axis cs:11303,0.733248116782226)
--(axis cs:9890,0.727132068285603)
--(axis cs:8477,0.720521533301611)
--(axis cs:7064,0.70771338187791)
--(axis cs:5651,0.688069453485247)
--(axis cs:4238,0.663119558026385)
--(axis cs:2825,0.61557799328187)
--(axis cs:1412,0.529997190504234)
--cycle;

\path [draw=violet, fill=violet, opacity=0.1]
(axis cs:0,0.749760993046473)
--(axis cs:0,0.609005964983663)
--(axis cs:0,0.749760993046473)
--(axis cs:0,0.749760993046473)
--cycle;

\path [draw=teal, fill=teal, opacity=0.1]
(axis cs:1412,0.476609593259657)
--(axis cs:1412,0.466754817707438)
--(axis cs:2825,0.570657427589623)
--(axis cs:4238,0.622236526262574)
--(axis cs:5651,0.650157783399472)
--(axis cs:7064,0.671570179896335)
--(axis cs:8477,0.685609934668474)
--(axis cs:9890,0.694852280316907)
--(axis cs:11303,0.702040282231584)
--(axis cs:12716,0.70455462006879)
--(axis cs:14129,0.706094602350398)
--(axis cs:14129,0.711004720750771)
--(axis cs:14129,0.711004720750771)
--(axis cs:12716,0.709214983155203)
--(axis cs:11303,0.704457725544761)
--(axis cs:9890,0.699499178007939)
--(axis cs:8477,0.687928583289134)
--(axis cs:7064,0.674711333888554)
--(axis cs:5651,0.654339619018891)
--(axis cs:4238,0.625208279242917)
--(axis cs:2825,0.577557353311195)
--(axis cs:1412,0.476609593259657)
--cycle;

\path [draw=cyan, fill=cyan, opacity=0.1]
(axis cs:1412,0.511972843725189)
--(axis cs:1412,0.503926788664869)
--(axis cs:2825,0.58459755464385)
--(axis cs:4238,0.621652329453262)
--(axis cs:5651,0.641085721433094)
--(axis cs:7064,0.656954072124422)
--(axis cs:8477,0.667235427292697)
--(axis cs:9890,0.672725714263196)
--(axis cs:11303,0.678769353763776)
--(axis cs:12716,0.680862180412569)
--(axis cs:14129,0.682866164301553)
--(axis cs:14129,0.686724454858849)
--(axis cs:14129,0.686724454858849)
--(axis cs:12716,0.685972213591565)
--(axis cs:11303,0.682005364722348)
--(axis cs:9890,0.677238320835677)
--(axis cs:8477,0.670430310666976)
--(axis cs:7064,0.659023393566179)
--(axis cs:5651,0.6449615370482)
--(axis cs:4238,0.62453268071314)
--(axis cs:2825,0.588191799033417)
--(axis cs:1412,0.511972843725189)
--cycle;

\addplot [thick, limegreen]
table {%
1412 0.514138997858196
2825 0.610406433613272
4238 0.657831756033621
5651 0.685682961145217
7064 0.705688893163615
8477 0.718438112300055
9890 0.72795823130589
11303 0.732905368409279
12716 0.737126794925616
14129 0.738903408311893
};
\addplot [thick, crimson]
table {%
1412 0.514663609594262
2825 0.609752589753959
4238 0.655263579743782
5651 0.683899783576316
7064 0.703279224388438
8477 0.716718706611104
9890 0.72466238965758
11303 0.731492275881194
12716 0.734575476464669
14129 0.73700244741974
};
\addplot [thick, coral]
table {%
0 0.679300085065007
};
\addplot [thick, gold]
table {%
1412 0.418296395108158
2825 0.539219722981708
4238 0.595704082160309
5651 0.628840959414856
7064 0.652588787004912
8477 0.669391413224706
9890 0.683665576115036
11303 0.693156193285373
12716 0.700043310402646
14129 0.704650513044356
};
\addplot [thick, purple]
table {%
1412 0.514193839077112
2825 0.607106415010111
4238 0.654818656319964
5651 0.683571215811378
7064 0.702787466619955
8477 0.717576322087316
9890 0.724517475252959
11303 0.731908784940703
12716 0.735021280592359
14129 0.737266805201648
};
\addplot [thick, blue]
table {%
1412 0.525204578093953
2825 0.613888988984209
4238 0.661001214507077
5651 0.685657333372688
7064 0.706209836442444
8477 0.717342003505137
9890 0.724627152000362
11303 0.730454765122789
12716 0.733896056247343
14129 0.735437245162152
};
\addplot [thick, violet]
table {%
0 0.679383479015068
};
\addplot [thick, teal]
table {%
1412 0.471682205483547
2825 0.574107390450409
4238 0.623722402752746
5651 0.652248701209181
7064 0.673140756892445
8477 0.686769258978804
9890 0.697175729162423
11303 0.703249003888172
12716 0.706884801611997
14129 0.708549661550585
};
\addplot [thick, cyan]
table {%
1412 0.507949816195029
2825 0.586394676838634
4238 0.623092505083201
5651 0.643023629240647
7064 0.6579887328453
8477 0.668832868979837
9890 0.674982017549437
11303 0.680387359243062
12716 0.683417197002067
14129 0.684795309580201
};
\end{axis}

\end{tikzpicture}


==> figures-results/allenoise_noisy_correct.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{coral}{RGB}{255,127,80}
\definecolor{crimson}{RGB}{220,20,60}
\definecolor{cyan}{RGB}{0,255,255}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{gold}{RGB}{255,215,0}
\definecolor{limegreen}{RGB}{50,205,50}
\definecolor{purple}{RGB}{128,0,128}
\definecolor{teal}{RGB}{0,128,128}
\definecolor{violet}{RGB}{238,130,238}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Step},
xmin=-706.45, xmax=14835.45,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Correct},
ymin=0.0511238628865083, ymax=0.11122070294625,
ytick style={color=black}
]
\path [draw=limegreen, fill=limegreen, opacity=0.1]
(axis cs:1412,0.0836798836231625)
--(axis cs:1412,0.0730062720675318)
--(axis cs:2825,0.0818720242870249)
--(axis cs:4238,0.0815959936009984)
--(axis cs:5651,0.0773547779027968)
--(axis cs:7064,0.0748581264295544)
--(axis cs:8477,0.0748871797510922)
--(axis cs:9890,0.071345849475413)
--(axis cs:11303,0.0716273127213306)
--(axis cs:12716,0.0692060766792403)
--(axis cs:14129,0.0682864201393025)
--(axis cs:14129,0.0738141836790644)
--(axis cs:14129,0.0738141836790644)
--(axis cs:12716,0.0751240677807804)
--(axis cs:11303,0.0756135426424796)
--(axis cs:9890,0.0778104940008281)
--(axis cs:8477,0.0792613922580595)
--(axis cs:7064,0.0810720986067742)
--(axis cs:5651,0.083464593640933)
--(axis cs:4238,0.0906100015768261)
--(axis cs:2825,0.0891699076894051)
--(axis cs:1412,0.0836798836231625)
--cycle;

\path [draw=crimson, fill=crimson, opacity=0.1]
(axis cs:1412,0.0899950761586975)
--(axis cs:1412,0.0706135518948587)
--(axis cs:2825,0.078554408564996)
--(axis cs:4238,0.0769078583896469)
--(axis cs:5651,0.079636464206534)
--(axis cs:7064,0.0750146712692361)
--(axis cs:8477,0.0736893431983628)
--(axis cs:9890,0.0709354226638983)
--(axis cs:11303,0.0723816091567087)
--(axis cs:12716,0.0718542106417292)
--(axis cs:14129,0.0715006092289674)
--(axis cs:14129,0.0751986654783365)
--(axis cs:14129,0.0751986654783365)
--(axis cs:12716,0.0759072662775949)
--(axis cs:11303,0.0762929687145557)
--(axis cs:9890,0.0781870911204688)
--(axis cs:8477,0.0779440666192432)
--(axis cs:7064,0.081948982086804)
--(axis cs:5651,0.0860817699438369)
--(axis cs:4238,0.0848583563175271)
--(axis cs:2825,0.0909445751807863)
--(axis cs:1412,0.0899950761586975)
--cycle;

\path [draw=coral, fill=coral, opacity=0.1]
(axis cs:0,0.0834454467222602)
--(axis cs:0,0.0741184145890846)
--(axis cs:0,0.0834454467222602)
--(axis cs:0,0.0834454467222602)
--cycle;

\path [draw=gold, fill=gold, opacity=0.1]
(axis cs:1412,0.0903978250423946)
--(axis cs:1412,0.0538555374346784)
--(axis cs:2825,0.0813477378727363)
--(axis cs:4238,0.0892100357605208)
--(axis cs:5651,0.0948082737474477)
--(axis cs:7064,0.0942556195812082)
--(axis cs:8477,0.0939110603017995)
--(axis cs:9890,0.0908779512139997)
--(axis cs:11303,0.088001633731711)
--(axis cs:12716,0.0885181719729169)
--(axis cs:14129,0.087391933028795)
--(axis cs:14129,0.0964190782512468)
--(axis cs:14129,0.0964190782512468)
--(axis cs:12716,0.0969375026432455)
--(axis cs:11303,0.0983631752237253)
--(axis cs:9890,0.102214524861477)
--(axis cs:8477,0.106462986910052)
--(axis cs:7064,0.10556051495806)
--(axis cs:5651,0.106268949192738)
--(axis cs:4238,0.104497919808568)
--(axis cs:2825,0.10848902839808)
--(axis cs:1412,0.0903978250423946)
--cycle;

\path [draw=purple, fill=purple, opacity=0.1]
(axis cs:1412,0.0851389866470493)
--(axis cs:1412,0.072893441096213)
--(axis cs:2825,0.0800237276741922)
--(axis cs:4238,0.0787148326289765)
--(axis cs:5651,0.0802325156146868)
--(axis cs:7064,0.0780229510169113)
--(axis cs:8477,0.0769220063830117)
--(axis cs:9890,0.0736713919602176)
--(axis cs:11303,0.073518953034701)
--(axis cs:12716,0.0724055858581036)
--(axis cs:14129,0.0730829570620593)
--(axis cs:14129,0.0796844420632166)
--(axis cs:14129,0.0796844420632166)
--(axis cs:12716,0.07877865477868)
--(axis cs:11303,0.0804354912772308)
--(axis cs:9890,0.0811438534524)
--(axis cs:8477,0.0817752101104628)
--(axis cs:7064,0.083444255274029)
--(axis cs:5651,0.0878321391009499)
--(axis cs:4238,0.0862612493652477)
--(axis cs:2825,0.0872261059961596)
--(axis cs:1412,0.0851389866470493)
--cycle;

\path [draw=blue, fill=blue, opacity=0.1]
(axis cs:1412,0.0849009027309064)
--(axis cs:1412,0.0762117182762267)
--(axis cs:2825,0.0796219659122578)
--(axis cs:4238,0.0792269244327724)
--(axis cs:5651,0.079257038050433)
--(axis cs:7064,0.0727925416965639)
--(axis cs:8477,0.072392303266862)
--(axis cs:9890,0.0728347058120512)
--(axis cs:11303,0.0704841170724036)
--(axis cs:12716,0.0699522824110394)
--(axis cs:14129,0.0690892937155655)
--(axis cs:14129,0.0751892820196046)
--(axis cs:14129,0.0751892820196046)
--(axis cs:12716,0.075978864270834)
--(axis cs:11303,0.0770816895898594)
--(axis cs:9890,0.076181043898347)
--(axis cs:8477,0.079256706898222)
--(axis cs:7064,0.0829491823579171)
--(axis cs:5651,0.0831236309150193)
--(axis cs:4238,0.0853147162400888)
--(axis cs:2825,0.0851981252360644)
--(axis cs:1412,0.0849009027309064)
--cycle;

\path [draw=violet, fill=violet, opacity=0.1]
(axis cs:0,0.0834545803959262)
--(axis cs:0,0.0734109958671573)
--(axis cs:0,0.0834545803959262)
--(axis cs:0,0.0834545803959262)
--cycle;

\path [draw=teal, fill=teal, opacity=0.1]
(axis cs:1412,0.0970221498887634)
--(axis cs:1412,0.0845150671167339)
--(axis cs:2825,0.0907520223185507)
--(axis cs:4238,0.0937161619047376)
--(axis cs:5651,0.0919172732754218)
--(axis cs:7064,0.09384101252458)
--(axis cs:8477,0.0924109208892129)
--(axis cs:9890,0.0912011111950558)
--(axis cs:11303,0.089426471891715)
--(axis cs:12716,0.0900395301812081)
--(axis cs:14129,0.0906800859770831)
--(axis cs:14129,0.100102659539793)
--(axis cs:14129,0.100102659539793)
--(axis cs:12716,0.0991595166130205)
--(axis cs:11303,0.102370014448475)
--(axis cs:9890,0.101661412649806)
--(axis cs:8477,0.104893432623311)
--(axis cs:7064,0.103892234346775)
--(axis cs:5651,0.108233116796874)
--(axis cs:4238,0.104676413256212)
--(axis cs:2825,0.102173281906598)
--(axis cs:1412,0.0970221498887634)
--cycle;

\path [draw=cyan, fill=cyan, opacity=0.1]
(axis cs:1412,0.0829015733458057)
--(axis cs:1412,0.0692181154180026)
--(axis cs:2825,0.0805586819565663)
--(axis cs:4238,0.0741926113908103)
--(axis cs:5651,0.0737090658079634)
--(axis cs:7064,0.0678032569133253)
--(axis cs:8477,0.0704442011957392)
--(axis cs:9890,0.067065038328243)
--(axis cs:11303,0.0664317576365022)
--(axis cs:12716,0.0673673147560171)
--(axis cs:14129,0.0662065781904044)
--(axis cs:14129,0.0727401100667063)
--(axis cs:14129,0.0727401100667063)
--(axis cs:12716,0.0726930692567137)
--(axis cs:11303,0.0763262708572336)
--(axis cs:9890,0.0739230537727505)
--(axis cs:8477,0.0750113926691883)
--(axis cs:7064,0.0783776006241195)
--(axis cs:5651,0.0838059842607659)
--(axis cs:4238,0.0817408789375282)
--(axis cs:2825,0.0843868943137131)
--(axis cs:1412,0.0829015733458057)
--cycle;

\addplot [thick, limegreen]
table {%
1412 0.0783430778453472
2825 0.085520965988215
4238 0.0861029975889122
5651 0.0804096857718649
7064 0.0779651125181643
8477 0.0770742860045759
9890 0.0745781717381205
11303 0.0736204276819051
12716 0.0721650722300104
14129 0.0710503019091835
};
\addplot [thick, crimson]
table {%
1412 0.0803043140267781
2825 0.0847494918728912
4238 0.080883107353587
5651 0.0828591170751854
7064 0.07848182667802
8477 0.075816704908803
9890 0.0745612568921836
11303 0.0743372889356322
12716 0.0738807384596621
14129 0.0733496373536519
};
\addplot [thick, coral]
table {%
0 0.0787819306556724
};
\addplot [thick, gold]
table {%
1412 0.0721266812385365
2825 0.0949183831354083
4238 0.0968539777845446
5651 0.100538611470093
7064 0.0999080672696339
8477 0.100187023605926
9890 0.0965462380377381
11303 0.0931824044777181
12716 0.0927278373080812
14129 0.0919055056400209
};
\addplot [thick, purple]
table {%
1412 0.0790162138716311
2825 0.0836249168351759
4238 0.0824880409971121
5651 0.0840323273578184
7064 0.0807336031454702
8477 0.0793486082467372
9890 0.0774076227063088
11303 0.0769772221559659
12716 0.0755921203183918
14129 0.0763836995626379
};
\addplot [thick, blue]
table {%
1412 0.0805563105035665
2825 0.0824100455741611
4238 0.0822708203364306
5651 0.0811903344827262
7064 0.0778708620272405
8477 0.075824505082542
9890 0.0745078748551991
11303 0.0737829033311315
12716 0.0729655733409367
14129 0.072139287867585
};
\addplot [thick, violet]
table {%
0 0.0784327881315418
};
\addplot [thick, teal]
table {%
1412 0.0907686085027486
2825 0.0964626521125743
4238 0.0991962875804748
5651 0.100075195036148
7064 0.0988666234356776
8477 0.0986521767562619
9890 0.0964312619224309
11303 0.0958982431700952
12716 0.0945995233971143
14129 0.0953913727584378
};
\addplot [thick, cyan]
table {%
1412 0.0760598443819042
2825 0.0824727881351397
4238 0.0779667451641692
5651 0.0787575250343647
7064 0.0730904287687224
8477 0.0727277969324637
9890 0.0704940460504967
11303 0.0713790142468679
12716 0.0700301920063654
14129 0.0694733441285554
};
\end{axis}

\end{tikzpicture}


==> figures-results/final/allenoise_noisy_correct.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{coral}{RGB}{255,127,80}
\definecolor{crimson}{RGB}{220,20,60}
\definecolor{cyan}{RGB}{0,255,255}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{gold}{RGB}{255,215,0}
\definecolor{limegreen}{RGB}{50,205,50}
\definecolor{purple}{RGB}{128,0,128}
\definecolor{teal}{RGB}{0,128,128}
\definecolor{violet}{RGB}{238,130,238}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Step},
xmin=-706.45, xmax=14835.45,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Correct noisy [\%]},
ymin=5.11238628865083, ymax=11.122070294625,
ytick style={color=black}
]
\path [draw=limegreen, fill=limegreen, opacity=0.1]
(axis cs:1412,8.36798836231625)
--(axis cs:1412,7.30062720675318)
--(axis cs:2825,8.18720242870249)
--(axis cs:4238,8.15959936009984)
--(axis cs:5651,7.73547779027968)
--(axis cs:7064,7.48581264295544)
--(axis cs:8477,7.48871797510922)
--(axis cs:9890,7.1345849475413)
--(axis cs:11303,7.16273127213306)
--(axis cs:12716,6.92060766792404)
--(axis cs:14129,6.82864201393025)
--(axis cs:14129,7.38141836790644)
--(axis cs:14129,7.38141836790644)
--(axis cs:12716,7.51240677807804)
--(axis cs:11303,7.56135426424796)
--(axis cs:9890,7.7810494000828)
--(axis cs:8477,7.92613922580595)
--(axis cs:7064,8.10720986067742)
--(axis cs:5651,8.3464593640933)
--(axis cs:4238,9.06100015768261)
--(axis cs:2825,8.91699076894051)
--(axis cs:1412,8.36798836231625)
--cycle;

\path [draw=crimson, fill=crimson, opacity=0.1]
(axis cs:1412,8.99950761586975)
--(axis cs:1412,7.06135518948587)
--(axis cs:2825,7.8554408564996)
--(axis cs:4238,7.69078583896469)
--(axis cs:5651,7.9636464206534)
--(axis cs:7064,7.50146712692361)
--(axis cs:8477,7.36893431983628)
--(axis cs:9890,7.09354226638983)
--(axis cs:11303,7.23816091567087)
--(axis cs:12716,7.18542106417292)
--(axis cs:14129,7.15006092289674)
--(axis cs:14129,7.51986654783365)
--(axis cs:14129,7.51986654783365)
--(axis cs:12716,7.59072662775949)
--(axis cs:11303,7.62929687145557)
--(axis cs:9890,7.81870911204688)
--(axis cs:8477,7.79440666192432)
--(axis cs:7064,8.1948982086804)
--(axis cs:5651,8.60817699438369)
--(axis cs:4238,8.48583563175271)
--(axis cs:2825,9.09445751807863)
--(axis cs:1412,8.99950761586975)
--cycle;

\path [draw=coral, fill=coral, opacity=0.1]
(axis cs:0,8.34454467222602)
--(axis cs:0,7.41184145890846)
--(axis cs:0,8.34454467222602)
--(axis cs:0,8.34454467222602)
--cycle;

\path [draw=gold, fill=gold, opacity=0.1]
(axis cs:1412,9.03978250423946)
--(axis cs:1412,5.38555374346784)
--(axis cs:2825,8.13477378727363)
--(axis cs:4238,8.92100357605208)
--(axis cs:5651,9.48082737474478)
--(axis cs:7064,9.42556195812082)
--(axis cs:8477,9.39110603017996)
--(axis cs:9890,9.08779512139997)
--(axis cs:11303,8.8001633731711)
--(axis cs:12716,8.85181719729169)
--(axis cs:14129,8.7391933028795)
--(axis cs:14129,9.64190782512468)
--(axis cs:14129,9.64190782512468)
--(axis cs:12716,9.69375026432455)
--(axis cs:11303,9.83631752237252)
--(axis cs:9890,10.2214524861477)
--(axis cs:8477,10.6462986910052)
--(axis cs:7064,10.556051495806)
--(axis cs:5651,10.6268949192738)
--(axis cs:4238,10.4497919808568)
--(axis cs:2825,10.848902839808)
--(axis cs:1412,9.03978250423946)
--cycle;

\path [draw=purple, fill=purple, opacity=0.1]
(axis cs:1412,8.51389866470493)
--(axis cs:1412,7.2893441096213)
--(axis cs:2825,8.00237276741922)
--(axis cs:4238,7.87148326289765)
--(axis cs:5651,8.02325156146869)
--(axis cs:7064,7.80229510169113)
--(axis cs:8477,7.69220063830117)
--(axis cs:9890,7.36713919602176)
--(axis cs:11303,7.3518953034701)
--(axis cs:12716,7.24055858581036)
--(axis cs:14129,7.30829570620593)
--(axis cs:14129,7.96844420632166)
--(axis cs:14129,7.96844420632166)
--(axis cs:12716,7.877865477868)
--(axis cs:11303,8.04354912772308)
--(axis cs:9890,8.11438534524)
--(axis cs:8477,8.17752101104628)
--(axis cs:7064,8.3444255274029)
--(axis cs:5651,8.78321391009499)
--(axis cs:4238,8.62612493652477)
--(axis cs:2825,8.72261059961596)
--(axis cs:1412,8.51389866470493)
--cycle;

\path [draw=blue, fill=blue, opacity=0.1]
(axis cs:1412,8.49009027309064)
--(axis cs:1412,7.62117182762267)
--(axis cs:2825,7.96219659122578)
--(axis cs:4238,7.92269244327724)
--(axis cs:5651,7.92570380504331)
--(axis cs:7064,7.27925416965639)
--(axis cs:8477,7.2392303266862)
--(axis cs:9890,7.28347058120512)
--(axis cs:11303,7.04841170724036)
--(axis cs:12716,6.99522824110394)
--(axis cs:14129,6.90892937155655)
--(axis cs:14129,7.51892820196046)
--(axis cs:14129,7.51892820196046)
--(axis cs:12716,7.5978864270834)
--(axis cs:11303,7.70816895898594)
--(axis cs:9890,7.6181043898347)
--(axis cs:8477,7.9256706898222)
--(axis cs:7064,8.29491823579171)
--(axis cs:5651,8.31236309150193)
--(axis cs:4238,8.53147162400888)
--(axis cs:2825,8.51981252360644)
--(axis cs:1412,8.49009027309064)
--cycle;

\path [draw=violet, fill=violet, opacity=0.1]
(axis cs:0,8.34545803959262)
--(axis cs:0,7.34109958671573)
--(axis cs:0,8.34545803959262)
--(axis cs:0,8.34545803959262)
--cycle;

\path [draw=teal, fill=teal, opacity=0.1]
(axis cs:1412,9.70221498887634)
--(axis cs:1412,8.45150671167339)
--(axis cs:2825,9.07520223185507)
--(axis cs:4238,9.37161619047376)
--(axis cs:5651,9.19172732754218)
--(axis cs:7064,9.384101252458)
--(axis cs:8477,9.24109208892129)
--(axis cs:9890,9.12011111950558)
--(axis cs:11303,8.9426471891715)
--(axis cs:12716,9.00395301812081)
--(axis cs:14129,9.06800859770831)
--(axis cs:14129,10.0102659539793)
--(axis cs:14129,10.0102659539793)
--(axis cs:12716,9.91595166130205)
--(axis cs:11303,10.2370014448475)
--(axis cs:9890,10.1661412649806)
--(axis cs:8477,10.4893432623311)
--(axis cs:7064,10.3892234346775)
--(axis cs:5651,10.8233116796874)
--(axis cs:4238,10.4676413256212)
--(axis cs:2825,10.2173281906598)
--(axis cs:1412,9.70221498887634)
--cycle;

\path [draw=cyan, fill=cyan, opacity=0.1]
(axis cs:1412,8.29015733458057)
--(axis cs:1412,6.92181154180026)
--(axis cs:2825,8.05586819565663)
--(axis cs:4238,7.41926113908103)
--(axis cs:5651,7.37090658079634)
--(axis cs:7064,6.78032569133253)
--(axis cs:8477,7.04442011957392)
--(axis cs:9890,6.70650383282429)
--(axis cs:11303,6.64317576365023)
--(axis cs:12716,6.73673147560172)
--(axis cs:14129,6.62065781904044)
--(axis cs:14129,7.27401100667063)
--(axis cs:14129,7.27401100667063)
--(axis cs:12716,7.26930692567137)
--(axis cs:11303,7.63262708572336)
--(axis cs:9890,7.39230537727505)
--(axis cs:8477,7.50113926691883)
--(axis cs:7064,7.83776006241195)
--(axis cs:5651,8.38059842607659)
--(axis cs:4238,8.17408789375282)
--(axis cs:2825,8.43868943137131)
--(axis cs:1412,8.29015733458057)
--cycle;

\addplot [thick, limegreen]
table {%
1412 7.83430778453472
2825 8.5520965988215
4238 8.61029975889122
5651 8.04096857718649
7064 7.79651125181643
8477 7.70742860045759
9890 7.45781717381205
11303 7.36204276819051
12716 7.21650722300104
14129 7.10503019091835
};
\addplot [thick, crimson]
table {%
1412 8.03043140267781
2825 8.47494918728912
4238 8.0883107353587
5651 8.28591170751854
7064 7.848182667802
8477 7.5816704908803
9890 7.45612568921836
11303 7.43372889356322
12716 7.38807384596621
14129 7.33496373536519
};
\addplot [thick, coral]
table {%
0 7.87819306556724
};
\addplot [thick, gold]
table {%
1412 7.21266812385365
2825 9.49183831354083
4238 9.68539777845446
5651 10.0538611470093
7064 9.99080672696339
8477 10.0187023605926
9890 9.65462380377381
11303 9.31824044777181
12716 9.27278373080812
14129 9.19055056400209
};
\addplot [thick, purple]
table {%
1412 7.90162138716311
2825 8.36249168351759
4238 8.24880409971121
5651 8.40323273578184
7064 8.07336031454702
8477 7.93486082467372
9890 7.74076227063088
11303 7.69772221559659
12716 7.55921203183918
14129 7.63836995626379
};
\addplot [thick, blue]
table {%
1412 8.05563105035665
2825 8.24100455741611
4238 8.22708203364306
5651 8.11903344827262
7064 7.78708620272405
8477 7.5824505082542
9890 7.45078748551991
11303 7.37829033311315
12716 7.29655733409367
14129 7.2139287867585
};
\addplot [thick, violet]
table {%
0 7.84327881315418
};
\addplot [thick, teal]
table {%
1412 9.07686085027486
2825 9.64626521125743
4238 9.91962875804748
5651 10.0075195036148
7064 9.88666234356776
8477 9.86521767562619
9890 9.64312619224309
11303 9.58982431700952
12716 9.45995233971143
14129 9.53913727584378
};
\addplot [thick, cyan]
table {%
1412 7.60598443819042
2825 8.24727881351397
4238 7.79667451641692
5651 7.87575250343647
7064 7.30904287687224
8477 7.27277969324637
9890 7.04940460504967
11303 7.13790142468679
12716 7.00301920063654
14129 6.94733441285554
};
\end{axis}

\end{tikzpicture}


==> figures-results/final/allenoise_noisy_memorized.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{coral}{RGB}{255,127,80}
\definecolor{crimson}{RGB}{220,20,60}
\definecolor{cyan}{RGB}{0,255,255}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{gold}{RGB}{255,215,0}
\definecolor{limegreen}{RGB}{50,205,50}
\definecolor{purple}{RGB}{128,0,128}
\definecolor{teal}{RGB}{0,128,128}
\definecolor{violet}{RGB}{238,130,238}

\begin{axis}[
tick align=outside,
tick pos=left,
title={AlleNoise},
x grid style={darkgray176},
xlabel={Step},
xmin=1312, xmax=14229,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Memorized [\%]},
ymin=28.7693354053335, ymax=74.0941652528341,
ytick style={color=black}
]
\path [draw=limegreen, fill=limegreen, opacity=0.1]
(axis cs:1412,45.803842462332)
--(axis cs:1412,44.8553119938094)
--(axis cs:2825,56.1671932857626)
--(axis cs:4238,61.3149568101193)
--(axis cs:5651,64.7358520550489)
--(axis cs:7064,66.4610927159072)
--(axis cs:8477,67.844767235532)
--(axis cs:9890,68.8967509435783)
--(axis cs:11303,69.5859295313863)
--(axis cs:12716,69.851501700875)
--(axis cs:14129,70.1625280767618)
--(axis cs:14129,71.1524095845398)
--(axis cs:14129,71.1524095845398)
--(axis cs:12716,71.0886060190323)
--(axis cs:11303,70.4506808282853)
--(axis cs:9890,69.6122649009314)
--(axis cs:8477,68.7292321709873)
--(axis cs:7064,67.586001911839)
--(axis cs:5651,65.4041344949872)
--(axis cs:4238,62.6854669553137)
--(axis cs:2825,56.9439763460329)
--(axis cs:1412,45.803842462332)
--cycle;

\path [draw=crimson, fill=crimson, opacity=0.1]
(axis cs:1412,45.4093935357286)
--(axis cs:1412,45.2678796140355)
--(axis cs:2825,56.4006332707984)
--(axis cs:4238,61.9225829164852)
--(axis cs:5651,63.8144632852188)
--(axis cs:7064,66.2687560417257)
--(axis cs:8477,67.9205303573167)
--(axis cs:9890,68.6806764874026)
--(axis cs:11303,69.4751792817768)
--(axis cs:12716,69.8830821288964)
--(axis cs:14129,70.0881632257707)
--(axis cs:14129,71.0306842168116)
--(axis cs:14129,71.0306842168116)
--(axis cs:12716,70.8212448739589)
--(axis cs:11303,70.3079938942348)
--(axis cs:9890,69.8065388776067)
--(axis cs:8477,69.1035681352954)
--(axis cs:7064,67.7083641431164)
--(axis cs:5651,65.5207999025713)
--(axis cs:4238,62.5134904997171)
--(axis cs:2825,57.2178313566)
--(axis cs:1412,45.4093935357286)
--cycle;

\path [draw=coral, fill=coral, opacity=0.1]
(axis cs:0,71.7611266170009)
--(axis cs:0,56.6070163029806)
--(axis cs:0,71.7611266170009)
--(axis cs:0,71.7611266170009)
--cycle;

\path [draw=gold, fill=gold, opacity=0.1]
(axis cs:1412,40.9476094631787)
--(axis cs:1412,30.8295549438562)
--(axis cs:2825,44.8912663820916)
--(axis cs:4238,52.4782555375729)
--(axis cs:5651,56.6939120581637)
--(axis cs:7064,59.4437393985013)
--(axis cs:8477,60.620997262287)
--(axis cs:9890,62.7798343517647)
--(axis cs:11303,64.00255765356)
--(axis cs:12716,65.0251363867595)
--(axis cs:14129,65.389444832777)
--(axis cs:14129,65.9605068753361)
--(axis cs:14129,65.9605068753361)
--(axis cs:12716,65.667628461696)
--(axis cs:11303,64.6311245976124)
--(axis cs:9890,63.7369409620617)
--(axis cs:8477,62.7121824068215)
--(axis cs:7064,60.4554171583328)
--(axis cs:5651,58.2580678701657)
--(axis cs:4238,54.5064597450888)
--(axis cs:2825,49.0350509669477)
--(axis cs:1412,40.9476094631787)
--cycle;

\path [draw=purple, fill=purple, opacity=0.1]
(axis cs:1412,45.2978484698725)
--(axis cs:1412,44.7837115939487)
--(axis cs:2825,55.8891690647766)
--(axis cs:4238,61.2796356133004)
--(axis cs:5651,64.2490708245243)
--(axis cs:7064,66.4548811838526)
--(axis cs:8477,67.6070551775161)
--(axis cs:9890,68.8969411601343)
--(axis cs:11303,69.4949683680431)
--(axis cs:12716,70.0095322312186)
--(axis cs:14129,70.0401214058971)
--(axis cs:14129,70.7202325129307)
--(axis cs:14129,70.7202325129307)
--(axis cs:12716,70.6264608964356)
--(axis cs:11303,70.2593805002348)
--(axis cs:9890,69.4675029006956)
--(axis cs:8477,68.7488997569106)
--(axis cs:7064,67.194431943717)
--(axis cs:5651,64.9004431250846)
--(axis cs:4238,62.3046774658715)
--(axis cs:2825,57.108092540434)
--(axis cs:1412,45.2978484698725)
--cycle;

\path [draw=blue, fill=blue, opacity=0.1]
(axis cs:1412,46.8018195896365)
--(axis cs:1412,46.0589056862998)
--(axis cs:2825,56.4581701284398)
--(axis cs:4238,61.9684087530309)
--(axis cs:5651,64.8619746717839)
--(axis cs:7064,66.8871014943747)
--(axis cs:8477,68.0833260015573)
--(axis cs:9890,69.1426500736171)
--(axis cs:11303,69.6263682488617)
--(axis cs:12716,69.8484371818153)
--(axis cs:14129,70.3206232362642)
--(axis cs:14129,70.3813349906967)
--(axis cs:14129,70.3813349906967)
--(axis cs:12716,70.3000947637017)
--(axis cs:11303,69.7854788684956)
--(axis cs:9890,69.3463996847676)
--(axis cs:8477,68.6883107995839)
--(axis cs:7064,67.3926271492096)
--(axis cs:5651,65.4755500735218)
--(axis cs:4238,62.3773197859666)
--(axis cs:2825,57.4127865910806)
--(axis cs:1412,46.8018195896365)
--cycle;

\path [draw=violet, fill=violet, opacity=0.1]
(axis cs:0,72.0339457143113)
--(axis cs:0,56.3452182983916)
--(axis cs:0,72.0339457143113)
--(axis cs:0,72.0339457143113)
--cycle;

\path [draw=teal, fill=teal, opacity=0.1]
(axis cs:1412,42.4069876417501)
--(axis cs:1412,40.8887951403309)
--(axis cs:2825,52.1477981005517)
--(axis cs:4238,57.1913442756438)
--(axis cs:5651,59.7987645224779)
--(axis cs:7064,62.3319685241067)
--(axis cs:8477,63.2647116797415)
--(axis cs:9890,64.3195272426802)
--(axis cs:11303,64.6802113972507)
--(axis cs:12716,65.1901402954395)
--(axis cs:14129,65.3390739053754)
--(axis cs:14129,66.1760903592036)
--(axis cs:14129,66.1760903592036)
--(axis cs:12716,65.9965618610887)
--(axis cs:11303,66.0177505033584)
--(axis cs:9890,64.9470020643677)
--(axis cs:8477,64.1179116094607)
--(axis cs:7064,62.7051745216096)
--(axis cs:5651,61.2772810143729)
--(axis cs:4238,58.0173710555925)
--(axis cs:2825,53.0992864382105)
--(axis cs:1412,42.4069876417501)
--cycle;

\path [draw=cyan, fill=cyan, opacity=0.1]
(axis cs:1412,45.7026628379225)
--(axis cs:1412,44.8527119890051)
--(axis cs:2825,54.2321104212177)
--(axis cs:4238,58.435805595477)
--(axis cs:5651,60.9365442389065)
--(axis cs:7064,62.5066530368306)
--(axis cs:8477,63.9207161833346)
--(axis cs:9890,64.4586702026597)
--(axis cs:11303,65.0724507525866)
--(axis cs:12716,65.2979016128295)
--(axis cs:14129,65.4994088740748)
--(axis cs:14129,66.7225625158563)
--(axis cs:14129,66.7225625158563)
--(axis cs:12716,66.6212439288605)
--(axis cs:11303,66.030499005447)
--(axis cs:9890,65.6624443239551)
--(axis cs:8477,64.7850821184027)
--(axis cs:7064,64.0843168559171)
--(axis cs:5651,62.556268848511)
--(axis cs:4238,60.1441571510465)
--(axis cs:2825,54.9289409167958)
--(axis cs:1412,45.7026628379225)
--cycle;

\addplot [thick, limegreen]
table {%
1412 45.3295772280707
2825 56.5555848158977
4238 62.0002118827165
5651 65.069993275018
7064 67.0235473138731
8477 68.2869997032596
9890 69.2545079222548
11303 70.0183051798358
12716 70.4700538599536
14129 70.6574688306508
};
\addplot [thick, crimson]
table {%
1412 45.338636574882
2825 56.8092323136992
4238 62.2180367081012
5651 64.6676315938951
7064 66.988560092421
8477 68.5120492463061
9890 69.2436076825046
11303 69.8915865880058
12716 70.3521635014276
14129 70.5594237212911
};
\addplot [thick, coral]
table {%
0 64.1840714599908
};
\addplot [thick, gold]
table {%
1412 35.8885822035175
2825 46.9631586745196
4238 53.4923576413309
5651 57.4759899641647
7064 59.949578278417
8477 61.6665898345543
9890 63.2583876569132
11303 64.3168411255862
12716 65.3463824242277
14129 65.6749758540566
};
\addplot [thick, purple]
table {%
1412 45.0407800319106
2825 56.4986308026053
4238 61.792156539586
5651 64.5747569748044
7064 66.8246565637848
8477 68.1779774672134
9890 69.182222030415
11303 69.8771744341389
12716 70.3179965638271
14129 70.3801769594139
};
\addplot [thick, blue]
table {%
1412 46.4303626379681
2825 56.9354783597602
4238 62.1728642694988
5651 65.1687623726528
7064 67.1398643217921
8477 68.3858184005706
9890 69.2445248791923
11303 69.7059235586786
12716 70.0742659727585
14129 70.3509791134804
};
\addplot [thick, violet]
table {%
0 64.1895820063515
};
\addplot [thick, teal]
table {%
1412 41.6478913910405
2825 52.6235422693811
4238 57.6043576656181
5651 60.5380227684254
7064 62.5185715228582
8477 63.6913116446011
9890 64.6332646535239
11303 65.3489809503046
12716 65.5933510782641
14129 65.7575821322895
};
\addplot [thick, cyan]
table {%
1412 45.2776874134638
2825 54.5805256690068
4238 59.2899813732617
5651 61.7464065437087
7064 63.2954849463738
8477 64.3528991508687
9890 65.0605572633074
11303 65.5514748790168
12716 65.959572770845
14129 66.1109856949655
};
\end{axis}

\end{tikzpicture}


==> figures-results/final/val_fraction_noisy_correct.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{coral}{RGB}{255,127,80}
\definecolor{crimson}{RGB}{220,20,60}
\definecolor{cyan}{RGB}{0,255,255}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{gold}{RGB}{255,215,0}
\definecolor{limegreen}{RGB}{50,205,50}
\definecolor{purple}{RGB}{128,0,128}
\definecolor{teal}{RGB}{0,128,128}
\definecolor{violet}{RGB}{238,130,238}

\begin{axis}[
tick align=outside,
tick pos=left,
title={AlleNoise},
x grid style={darkgray176},
xlabel={Step},
xmin=1312, xmax=14229,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Correct noisy [\%]},
ymin=5.11238628865083, ymax=11.122070294625,
ytick style={color=black}
]
\path [draw=limegreen, fill=limegreen, opacity=0.1]
(axis cs:1412,8.36798836231625)
--(axis cs:1412,7.30062720675318)
--(axis cs:2825,8.18720242870249)
--(axis cs:4238,8.15959936009984)
--(axis cs:5651,7.73547779027968)
--(axis cs:7064,7.48581264295544)
--(axis cs:8477,7.48871797510922)
--(axis cs:9890,7.1345849475413)
--(axis cs:11303,7.16273127213306)
--(axis cs:12716,6.92060766792404)
--(axis cs:14129,6.82864201393025)
--(axis cs:14129,7.38141836790644)
--(axis cs:14129,7.38141836790644)
--(axis cs:12716,7.51240677807804)
--(axis cs:11303,7.56135426424796)
--(axis cs:9890,7.7810494000828)
--(axis cs:8477,7.92613922580595)
--(axis cs:7064,8.10720986067742)
--(axis cs:5651,8.3464593640933)
--(axis cs:4238,9.06100015768261)
--(axis cs:2825,8.91699076894051)
--(axis cs:1412,8.36798836231625)
--cycle;

\path [draw=crimson, fill=crimson, opacity=0.1]
(axis cs:1412,8.99950761586975)
--(axis cs:1412,7.06135518948587)
--(axis cs:2825,7.8554408564996)
--(axis cs:4238,7.69078583896469)
--(axis cs:5651,7.9636464206534)
--(axis cs:7064,7.50146712692361)
--(axis cs:8477,7.36893431983628)
--(axis cs:9890,7.09354226638983)
--(axis cs:11303,7.23816091567087)
--(axis cs:12716,7.18542106417292)
--(axis cs:14129,7.15006092289674)
--(axis cs:14129,7.51986654783365)
--(axis cs:14129,7.51986654783365)
--(axis cs:12716,7.59072662775949)
--(axis cs:11303,7.62929687145557)
--(axis cs:9890,7.81870911204688)
--(axis cs:8477,7.79440666192432)
--(axis cs:7064,8.1948982086804)
--(axis cs:5651,8.60817699438369)
--(axis cs:4238,8.48583563175271)
--(axis cs:2825,9.09445751807863)
--(axis cs:1412,8.99950761586975)
--cycle;

\path [draw=coral, fill=coral, opacity=0.1]
(axis cs:0,8.34454467222602)
--(axis cs:0,7.41184145890846)
--(axis cs:0,8.34454467222602)
--(axis cs:0,8.34454467222602)
--cycle;

\path [draw=gold, fill=gold, opacity=0.1]
(axis cs:1412,9.03978250423946)
--(axis cs:1412,5.38555374346784)
--(axis cs:2825,8.13477378727363)
--(axis cs:4238,8.92100357605208)
--(axis cs:5651,9.48082737474478)
--(axis cs:7064,9.42556195812082)
--(axis cs:8477,9.39110603017996)
--(axis cs:9890,9.08779512139997)
--(axis cs:11303,8.8001633731711)
--(axis cs:12716,8.85181719729169)
--(axis cs:14129,8.7391933028795)
--(axis cs:14129,9.64190782512468)
--(axis cs:14129,9.64190782512468)
--(axis cs:12716,9.69375026432455)
--(axis cs:11303,9.83631752237252)
--(axis cs:9890,10.2214524861477)
--(axis cs:8477,10.6462986910052)
--(axis cs:7064,10.556051495806)
--(axis cs:5651,10.6268949192738)
--(axis cs:4238,10.4497919808568)
--(axis cs:2825,10.848902839808)
--(axis cs:1412,9.03978250423946)
--cycle;

\path [draw=purple, fill=purple, opacity=0.1]
(axis cs:1412,8.51389866470493)
--(axis cs:1412,7.2893441096213)
--(axis cs:2825,8.00237276741922)
--(axis cs:4238,7.87148326289765)
--(axis cs:5651,8.02325156146869)
--(axis cs:7064,7.80229510169113)
--(axis cs:8477,7.69220063830117)
--(axis cs:9890,7.36713919602176)
--(axis cs:11303,7.3518953034701)
--(axis cs:12716,7.24055858581036)
--(axis cs:14129,7.30829570620593)
--(axis cs:14129,7.96844420632166)
--(axis cs:14129,7.96844420632166)
--(axis cs:12716,7.877865477868)
--(axis cs:11303,8.04354912772308)
--(axis cs:9890,8.11438534524)
--(axis cs:8477,8.17752101104628)
--(axis cs:7064,8.3444255274029)
--(axis cs:5651,8.78321391009499)
--(axis cs:4238,8.62612493652477)
--(axis cs:2825,8.72261059961596)
--(axis cs:1412,8.51389866470493)
--cycle;

\path [draw=blue, fill=blue, opacity=0.1]
(axis cs:1412,8.49009027309064)
--(axis cs:1412,7.62117182762267)
--(axis cs:2825,7.96219659122578)
--(axis cs:4238,7.92269244327724)
--(axis cs:5651,7.92570380504331)
--(axis cs:7064,7.27925416965639)
--(axis cs:8477,7.2392303266862)
--(axis cs:9890,7.28347058120512)
--(axis cs:11303,7.04841170724036)
--(axis cs:12716,6.99522824110394)
--(axis cs:14129,6.90892937155655)
--(axis cs:14129,7.51892820196046)
--(axis cs:14129,7.51892820196046)
--(axis cs:12716,7.5978864270834)
--(axis cs:11303,7.70816895898594)
--(axis cs:9890,7.6181043898347)
--(axis cs:8477,7.9256706898222)
--(axis cs:7064,8.29491823579171)
--(axis cs:5651,8.31236309150193)
--(axis cs:4238,8.53147162400888)
--(axis cs:2825,8.51981252360644)
--(axis cs:1412,8.49009027309064)
--cycle;

\path [draw=violet, fill=violet, opacity=0.1]
(axis cs:0,8.34545803959262)
--(axis cs:0,7.34109958671573)
--(axis cs:0,8.34545803959262)
--(axis cs:0,8.34545803959262)
--cycle;

\path [draw=teal, fill=teal, opacity=0.1]
(axis cs:1412,9.70221498887634)
--(axis cs:1412,8.45150671167339)
--(axis cs:2825,9.07520223185507)
--(axis cs:4238,9.37161619047376)
--(axis cs:5651,9.19172732754218)
--(axis cs:7064,9.384101252458)
--(axis cs:8477,9.24109208892129)
--(axis cs:9890,9.12011111950558)
--(axis cs:11303,8.9426471891715)
--(axis cs:12716,9.00395301812081)
--(axis cs:14129,9.06800859770831)
--(axis cs:14129,10.0102659539793)
--(axis cs:14129,10.0102659539793)
--(axis cs:12716,9.91595166130205)
--(axis cs:11303,10.2370014448475)
--(axis cs:9890,10.1661412649806)
--(axis cs:8477,10.4893432623311)
--(axis cs:7064,10.3892234346775)
--(axis cs:5651,10.8233116796874)
--(axis cs:4238,10.4676413256212)
--(axis cs:2825,10.2173281906598)
--(axis cs:1412,9.70221498887634)
--cycle;

\path [draw=cyan, fill=cyan, opacity=0.1]
(axis cs:1412,8.29015733458057)
--(axis cs:1412,6.92181154180026)
--(axis cs:2825,8.05586819565663)
--(axis cs:4238,7.41926113908103)
--(axis cs:5651,7.37090658079634)
--(axis cs:7064,6.78032569133253)
--(axis cs:8477,7.04442011957392)
--(axis cs:9890,6.70650383282429)
--(axis cs:11303,6.64317576365023)
--(axis cs:12716,6.73673147560172)
--(axis cs:14129,6.62065781904044)
--(axis cs:14129,7.27401100667063)
--(axis cs:14129,7.27401100667063)
--(axis cs:12716,7.26930692567137)
--(axis cs:11303,7.63262708572336)
--(axis cs:9890,7.39230537727505)
--(axis cs:8477,7.50113926691883)
--(axis cs:7064,7.83776006241195)
--(axis cs:5651,8.38059842607659)
--(axis cs:4238,8.17408789375282)
--(axis cs:2825,8.43868943137131)
--(axis cs:1412,8.29015733458057)
--cycle;

\addplot [thick, limegreen]
table {%
1412 7.83430778453472
2825 8.5520965988215
4238 8.61029975889122
5651 8.04096857718649
7064 7.79651125181643
8477 7.70742860045759
9890 7.45781717381205
11303 7.36204276819051
12716 7.21650722300104
14129 7.10503019091835
};
\addplot [thick, crimson]
table {%
1412 8.03043140267781
2825 8.47494918728912
4238 8.0883107353587
5651 8.28591170751854
7064 7.848182667802
8477 7.5816704908803
9890 7.45612568921836
11303 7.43372889356322
12716 7.38807384596621
14129 7.33496373536519
};
\addplot [thick, coral]
table {%
0 7.87819306556724
};
\addplot [thick, gold]
table {%
1412 7.21266812385365
2825 9.49183831354083
4238 9.68539777845446
5651 10.0538611470093
7064 9.99080672696339
8477 10.0187023605926
9890 9.65462380377381
11303 9.31824044777181
12716 9.27278373080812
14129 9.19055056400209
};
\addplot [thick, purple]
table {%
1412 7.90162138716311
2825 8.36249168351759
4238 8.24880409971121
5651 8.40323273578184
7064 8.07336031454702
8477 7.93486082467372
9890 7.74076227063088
11303 7.69772221559659
12716 7.55921203183918
14129 7.63836995626379
};
\addplot [thick, blue]
table {%
1412 8.05563105035665
2825 8.24100455741611
4238 8.22708203364306
5651 8.11903344827262
7064 7.78708620272405
8477 7.5824505082542
9890 7.45078748551991
11303 7.37829033311315
12716 7.29655733409367
14129 7.2139287867585
};
\addplot [thick, violet]
table {%
0 7.84327881315418
};
\addplot [thick, teal]
table {%
1412 9.07686085027486
2825 9.64626521125743
4238 9.91962875804748
5651 10.0075195036148
7064 9.88666234356776
8477 9.86521767562619
9890 9.64312619224309
11303 9.58982431700952
12716 9.45995233971143
14129 9.53913727584378
};
\addplot [thick, cyan]
table {%
1412 7.60598443819042
2825 8.24727881351397
4238 7.79667451641692
5651 7.87575250343647
7064 7.30904287687224
8477 7.27277969324637
9890 7.04940460504967
11303 7.13790142468679
12716 7.00301920063654
14129 6.94733441285554
};
\end{axis}

\end{tikzpicture}


==> plot_nest15_memorized.tex <==
\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=776.15, xmax=14764.85,
xtick style={color=black},
y grid style={darkgray176},
ymin=0.0123345112524268, ymax=0.0398595848252366,
ytick style={color=black},
width=6cm,
at={($ (nested_memorized.west)+(2cm,-1.2cm) $)}
]
\path [draw=springgreen, fill=springgreen, opacity=0.1]
(axis cs:1412,0.0217278369598006)
--(axis cs:1412,0.0162310208189914)
--(axis cs:2825,0.0167505897728258)
--(axis cs:4238,0.0189752038033979)
--(axis cs:5651,0.0195967908643778)
--(axis cs:7064,0.0218436496242904)
--(axis cs:8477,0.0239521190308819)
--(axis cs:9890,0.0263937280767216)
--(axis cs:11303,0.0275019054091955)
--(axis cs:12716,0.0317236070001005)
--(axis cs:14129,0.0316354270229327)
--(axis cs:14129,0.0348587466738656)
--(axis cs:14129,0.0348587466738656)
--(axis cs:12716,0.0349033357478015)
--(axis cs:11303,0.0339489931077524)
--(axis cs:9890,0.0310088539119382)
--(axis cs:8477,0.0266153726007263)
--(axis cs:7064,0.0247420696489335)
--(axis cs:5651,0.0215473350657294)
--(axis cs:4238,0.0213724179196402)
--(axis cs:2825,0.0198146278626122)
--(axis cs:1412,0.0217278369598006)
--cycle;

\path [draw=crimson, fill=crimson, opacity=0.1]
(axis cs:1412,0.0217278369598006)
--(axis cs:1412,0.0162310208189914)
--(axis cs:2825,0.0161225361803575)
--(axis cs:4238,0.0193012634653193)
--(axis cs:5651,0.0205067050777827)
--(axis cs:7064,0.0216148726824848)
--(axis cs:8477,0.0238301108141362)
--(axis cs:9890,0.0264135065528692)
--(axis cs:11303,0.0276757957608057)
--(axis cs:12716,0.0292344920814192)
--(axis cs:14129,0.0315041386337166)
--(axis cs:14129,0.0359854781526777)
--(axis cs:14129,0.0359854781526777)
--(axis cs:12716,0.0365960015091902)
--(axis cs:11303,0.0331113896200875)
--(axis cs:9890,0.0321173976760436)
--(axis cs:8477,0.0284627949541884)
--(axis cs:7064,0.0243072655741482)
--(axis cs:5651,0.0228937130142602)
--(axis cs:4238,0.0221081032982018)
--(axis cs:2825,0.0199118364597273)
--(axis cs:1412,0.0217278369598006)
--cycle;

\path [draw=purple, fill=purple, opacity=0.1]
(axis cs:1412,0.0195719760951228)
--(axis cs:1412,0.0165949894367807)
--(axis cs:2825,0.0153723073744508)
--(axis cs:4238,0.0136540047860792)
--(axis cs:5651,0.0156022542142062)
--(axis cs:7064,0.0142474499393731)
--(axis cs:8477,0.0143843260391727)
--(axis cs:9890,0.0145842289074692)
--(axis cs:11303,0.0158253575344517)
--(axis cs:12716,0.0155596349427526)
--(axis cs:14129,0.015880880917748)
--(axis cs:14129,0.0184281326353968)
--(axis cs:14129,0.0184281326353968)
--(axis cs:12716,0.0176211994995584)
--(axis cs:11303,0.0177536079018855)
--(axis cs:9890,0.0173357014127255)
--(axis cs:8477,0.0179338673945118)
--(axis cs:7064,0.0169423551943268)
--(axis cs:5651,0.0179766341524437)
--(axis cs:4238,0.0172040263542581)
--(axis cs:2825,0.0181403230811334)
--(axis cs:1412,0.0195719760951228)
--cycle;

\path [draw=blue, fill=blue, opacity=0.1]
(axis cs:1412,0.0210549934568065)
--(axis cs:1412,0.0135856509602818)
--(axis cs:2825,0.0158099760967811)
--(axis cs:4238,0.0178658009046784)
--(axis cs:5651,0.0174088078558133)
--(axis cs:7064,0.0234971507847566)
--(axis cs:8477,0.0256564674483425)
--(axis cs:9890,0.0288540247552255)
--(axis cs:11303,0.030539615506807)
--(axis cs:12716,0.0333212083308564)
--(axis cs:14129,0.0337255409962021)
--(axis cs:14129,0.0386084451173816)
--(axis cs:14129,0.0386084451173816)
--(axis cs:12716,0.0376855056499922)
--(axis cs:11303,0.0352246532026027)
--(axis cs:9890,0.0321985335785454)
--(axis cs:8477,0.0302201127142062)
--(axis cs:7064,0.0268048577944207)
--(axis cs:5651,0.0241999381884473)
--(axis cs:4238,0.0223490737871666)
--(axis cs:2825,0.0192286671948696)
--(axis cs:1412,0.0210549934568065)
--cycle;

\path [draw=teal, fill=teal, opacity=0.1]
(axis cs:1412,0.0203713768097478)
--(axis cs:1412,0.0157292647513581)
--(axis cs:2825,0.0159168079583932)
--(axis cs:4238,0.0149218928106417)
--(axis cs:5651,0.0150203123924541)
--(axis cs:7064,0.0165183337166961)
--(axis cs:8477,0.0173992323419801)
--(axis cs:9890,0.0180319400599135)
--(axis cs:11303,0.0186233314514143)
--(axis cs:12716,0.0195807022209121)
--(axis cs:14129,0.0201302130661869)
--(axis cs:14129,0.023801149110807)
--(axis cs:14129,0.023801149110807)
--(axis cs:12716,0.0230897338140549)
--(axis cs:11303,0.0227199535603261)
--(axis cs:9890,0.0207232237467521)
--(axis cs:8477,0.0180377621428029)
--(axis cs:7064,0.0189188259174165)
--(axis cs:5651,0.0180941870691039)
--(axis cs:4238,0.0164007804637597)
--(axis cs:2825,0.0179938544016193)
--(axis cs:1412,0.0203713768097478)
--cycle;

\path [draw=cyan, fill=cyan, opacity=0.1]
(axis cs:1412,0.0236132018084307)
--(axis cs:1412,0.0172012530297784)
--(axis cs:2825,0.0160749057722674)
--(axis cs:4238,0.0170089126756517)
--(axis cs:5651,0.0220062227033706)
--(axis cs:7064,0.0224999848244651)
--(axis cs:8477,0.0243908655106622)
--(axis cs:9890,0.0258372082375305)
--(axis cs:11303,0.0293210285108383)
--(axis cs:12716,0.030719652228289)
--(axis cs:14129,0.028777692437155)
--(axis cs:14129,0.0331377601342144)
--(axis cs:14129,0.0331377601342144)
--(axis cs:12716,0.032105318071439)
--(axis cs:11303,0.0331722852350505)
--(axis cs:9890,0.0296878497418116)
--(axis cs:8477,0.0294751757024631)
--(axis cs:7064,0.0281584894078537)
--(axis cs:5651,0.0277673814205475)
--(axis cs:4238,0.0220355633967242)
--(axis cs:2825,0.0238546239077645)
--(axis cs:1412,0.0236132018084307)
--cycle;

\addplot [semithick, springgreen]
table {%
1412 0.018979428889396
2825 0.018282608817719
4238 0.0201738108615191
5651 0.0205720629650536
7064 0.023292859636612
8477 0.0252837458158041
9890 0.0287012909943299
11303 0.030725449258474
12716 0.033313471373951
14129 0.0332470868483992
};
\addplot [semithick, crimson]
table {%
1412 0.018979428889396
2825 0.0180171863200424
4238 0.0207046833817606
5651 0.0217002090460214
7064 0.0229610691283165
8477 0.0261464528841623
9890 0.0292654521144564
11303 0.0303935926904466
12716 0.0329152467953047
14129 0.0337448083931972
};
\addplot [semithick, purple]
table {%
1412 0.0180834827659518
2825 0.0167563152277921
4238 0.0154290155701686
5651 0.016789444183325
7064 0.0155949025668499
8477 0.0161590967168423
9890 0.0159599651600974
11303 0.0167894827181686
12716 0.0165904172211555
14129 0.0171545067765724
};
\addplot [semithick, blue]
table {%
1412 0.0173203222085441
2825 0.0175193216458254
4238 0.0201074373459225
5651 0.0208043730221303
7064 0.0251510042895886
8477 0.0279382900812744
9890 0.0305262791668855
11303 0.0328821343547049
12716 0.0355033569904243
14129 0.0361669930567919
};
\addplot [semithick, teal]
table {%
1412 0.018050320780553
2825 0.0169553311800062
4238 0.0156613366372007
5651 0.016557249730779
7064 0.0177185798170563
8477 0.0177184972423915
9890 0.0193775819033328
11303 0.0206716425058702
12716 0.0213352180174835
14129 0.021965681088497
};
\addplot [semithick, cyan]
table {%
1412 0.0204072274191046
2825 0.0199647648400159
4238 0.019522238036188
5651 0.0248868020619591
7064 0.0253292371161594
8477 0.0269330206065626
9890 0.027762528989671
11303 0.0312466568729444
12716 0.031412485149864
14129 0.0309577262856847
};
\end{axis}



==> results_noise_type_1 <==

\begin{figure}[h]
    \centering
    % \resizebox{\textwidth}{!}{
    %     \input{plot_grid}
    % }
    \includegraphics[width=\textwidth]{figures-results/full_15.png}
    \caption{Validation accuracy, validation accuracy for noisy observations (with respect to clean labels) (noisy correct), and validation fraction of noisy instances for which the noisy label was predicted (memorized fraction). Level of noise is 15\%. We plot mean values and standard deviations from 5 cross-validation runs. Memorized fraction for symmetric and pair-flip noises in negligibly close to zero. For the plots for which zoomed view is meaningful we insert zoomed-in plots. Symmetric and pair-flip noises are not memorized at all, and the fraction memorized is around zero. CCE is hidden behind CE plot.}
    % \caption{Validation accuracy and fraction of noisy validation samples for which model predicts the noisy class. Level of noise is 15\%. We plot mean values and standard deviations from 5 cross-validation runs. All plots share y-scale. Fraction memorized for symmetric and pair-flip noises in negligibly close to zero. For the plots for which zoomed view is meaningful we insert zoomed-in plots. Symmetric and pair-flip noises are not memorized at all, and the fraction memorized is around zero. CCE is hidden behind CE plot.}
    \label{fig:validation-plots}
\end{figure}


% można powiedzieć, że metryka val_fraction_noisy_memorized mierzy memoryzację w klasach, które zostały zaszumione, a nie memoryzację tych konkretnych instancji, które zostały zaszumione

Figure~\ref{fig:validation-plots} shows plots of these metrics  for various noise types and methods. 


Noise in the data harms the performance also because 


\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figures-results/elr_plots_selected_15.png}
    \caption{We follow\cite{liu_early-learning_2020} and plot TODO}
    \label{fig:elr-like-plots}
\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figures-results/elr_15.png}
    \caption{We follow\cite{liu_early-learning_2020} and plot TODO}
    \label{fig:elr-like-plots-full}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
--------------------------------------------------------

% To understand the difference between synthetic noises and AlleNoise better, we delve into validation metrics. We compute validation accuracy (with respect to clean labels) and fraction of noisy observations for which the noisy class, which is incorrect, was predicted (memorized fraction). Figure~\ref{fig:validation-plots} shows plots of those two metrics  for various noise types and methods.

A noise in the data is harmful in many ways. On one hand, it reduces the number of clean observations that provide signal for training a classifier, while on the other, it confuses the classifier which learns to predict an incorrect label. Symmetric noise and pair-flip noise are not memorized at all by baseline cross-entropy. What seems to harm the performance of SPL on pair-flip noise is not memorization (fraction of memorized noisy examples is zero), but removal of training examples. Baseline cross-entropy does nothing to prevent memorization and uses all the observations, and performs  quite well. Moreover, ELR which does not remove observations, but smoothly corrects the targets is not only robust to memorization of this noise, but outperforms all other methods. Robustness of ELR to synthetic noise is also visible on zoomed-in plots of memorized fraction of nested-flip and matrix-flip noises. 

% Surprisingly, all methods based on filtration of noisy instances (CCE, CT, CTP, PRL, SPL) performed poorly on synthetic noise. Noise filtration is only effective if the filtering criterion is well suited to the noise distribution. Otherwise, it leads to loss of both clean and noisy training instances. This is the case for CT and SPL, which are outperformed by simplistic loss clipping implemented in CCE (and in some cases by the baseline CE). These methods excel on benchmarks like CIFAR-10, but their filtering criteria turn out to be inadequate for an unbalanced dataset with many classes.


The story of AlleNoise is different. SPL and PRL seem to correctly remove some of incorrectly labelled training observations, as the memorized fraction is lower than for the other methods, but this could be as well (or even more likely) due to the fact that the model has not managed to learn as much as other models (what is visible on accuracy plot). All in all, on AlleNoise we observe extreme memorization of incorrect training classes. Surely it is a significant, but not necessary only, factor leading to low accuracy of all methods. 

In general, we observe that the more instance-dependent and realistic is the noise, the harder it is to avoid its memorization. 

TODO skomentowac przyblizony wykres

TODO wrzucic tikzowy gdy bedzie komplet wynikow


==> table-pretrained-noise-15-and-40-version2.tex <==
\begin{table}[]
\begin{tabular}{lrrrrrrrrrr}
\multicolumn{1}{c}{\multirow{3}{*}{}} & \multicolumn{1}{c}{\multirow{3}{*}{Clean set}} & \multicolumn{8}{c}{Synthetic}                                                                                                                                                                                                                                                                                                                                                                         & \multicolumn{1}{c}{\multirow{3}{*}{AlleNoise}} \\
\multicolumn{1}{c}{}                  & \multicolumn{1}{c}{}                           & \multicolumn{4}{c}{Noise level 15\%}                                                                                                                                                & \multicolumn{4}{c}{Noise level 40\%}                                                                                                                                                                            & \multicolumn{1}{c}{}                                 \\
\multicolumn{1}{c}{}                  & \multicolumn{1}{c}{}                           & \multicolumn{1}{c}{Sym} & \multicolumn{1}{c}{PF} & \multicolumn{1}{c}{NF} & \multicolumn{1}{c}{MF} & \multicolumn{1}{c}{Sym}                                        & \multicolumn{1}{c}{PF} & \multicolumn{1}{c}{NF} & \multicolumn{1}{c}{MF} & \multicolumn{1}{c}{}                                 \\

CE                                    & 74.85  & 71.986  & 71.915  & 71.766  & 70.66  & 67.29  & 55.18  & 52.87  & 53.97  & 63.71                                          \\
ELR                                   & 74.81  & 72.15  & 73.21  & 73.07  & []  & 67.23  & 66.12  & 62.27  & []  & 63.72                                         \\
Mixup                                 & []  & []  & []  & []  & []  & []  & []  & []  & []  & [] ± []                                      \\
CCE                                   & 74.800  & 73.01  & 71.86  & 71.62  & []  & 68.73 & 55.13  & 52.07  & []  & 63.73                                         \\
CT                                    & 74.85  & []  & []  & []  & []  & []  & []  & []  & []  & [] ± []                                      \\
CT+                                   & 74.85  & []  & []  & []  & []  & []  & []  & []  & []  & [] ± []                                      \\
PRL                                   & 74.85  & 71.82  & 71.95  & 71.73  & []  & 65.01  & 62.22  & 56.39  & []  & 61.66                                         \\
SPL                                   & 74.85  & 72.56  & 68.29  & 67.57  & []  & 65.27  & 44.92  & 42.29  & []  & 59.10                                         \\
GJSD                                  & 74.63  & 73.28  & []  & []  & []  & []  & []  & []  & []  & 63.63                                        
\end{tabular}
\end{table}

==> table-pretrained-noise15-and-40.tex <==
\begin{table}[]
\begin{tabular}{lllllllllll}
\multicolumn{2}{l}{} & CE & ELR & Mixup & CCE & CT & CT+ & PRL & SPL & GJSD \\
\multicolumn{2}{l}{Clean set} & 74.85 ± 0.15 & 74.81 ± 0.11 & {[}{]} ± {[}{]} & 74.80 ± 0.09 & 74.85 ± 0.15 & 74.85 ± 0.15 & 74.85 ± 0.15 & 74.85 ± 0.15 & 74.63 ± 0.10 \\
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Synthetic\\ 15\%\end{tabular}} & Sym. & 71.99 ± 0.08 & 72.15 ± 0.10 & {[}{]} ± {[}{]} & 73.01 ± 0.10 & {[}{]} ± {[}{]} & {[}{]} ± {[}{]} & 71.82 ± 0.17 & 72.56 ± 0.10 & 73.28 ± 0.13 \\
 & PF & 71.92 ± 0.08 & 73.21 ± 0.21 & {[}{]} ± {[}{]} & 71.86 ± 0.17 & {[}{]} ± {[}{]} & {[}{]} ± {[}{]} & 71.95 ± 0.15 & 68.29 ± 0.15 & {[}{]} ± {[}{]} \\
 & NF & 71.77 ± 0.08 & 73.07 ± 0.11 & {[}{]} ± {[}{]} & 71.62 ± 0.10 & {[}{]} ± {[}{]} & {[}{]} ± {[}{]} & 71.73 ± 0.16 & 67.57 ± 0.14 & {[}{]} ± {[}{]} \\
 & MF & 70.66 ± 0.12 & {[}{]} ± {[}{]} & {[}{]} ± {[}{]} & {[}{]} ± {[}{]} & {[}{]} ± {[}{]} & {[}{]} ± {[}{]} & {[}{]} ± {[}{]} & {[}{]} ± {[}{]} & {[}{]} ± {[}{]} \\
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Synthetic\\ 40\%\end{tabular}} & Sym. & 67.29 ± 0.12 & 67.23 ± 0.18 & {[}{]} ± {[}{]} & 68.73 ± 0.06 & {[}{]} ± {[}{]} & {[}{]} ± {[}{]} & 65.01 ± 0.30 & 65.27 ± 0.35 & {[}{]} ± {[}{]} \\
 & PF & 55.18 ± 0.26 & 66.12 ± 0.15 & {[}{]} ± {[}{]} & 55.13 ± 0.28 & {[}{]} ± {[}{]} & {[}{]} ± {[}{]} & 62.22 ± 0.45 & 44.92 ± 1.52 & {[}{]} ± {[}{]} \\
 & NF & 52.87 ± 0.19 & 62.27 ± 0.19 & {[}{]} ± {[}{]} & 52.07 ± 0.58 & {[}{]} ± {[}{]} & {[}{]} ± {[}{]} & 56.39 ± 0.40 & 42.29 ± 1.06 & {[}{]} ± {[}{]} \\
 & MF & 53.97 ± 0.26 & {[}{]} ± {[}{]} & {[}{]} ± {[}{]} & {[}{]} ± {[}{]} & {[}{]} ± {[}{]} & {[}{]} ± {[}{]} & {[}{]} ± {[}{]} & {[}{]} ± {[}{]} & {[}{]} ± {[}{]} \\
\multicolumn{2}{l}{AlleNoise 15\%} & 63.71 ± 0.11 & 63.72 ± 0.19 & {[}{]} ± {[}{]} & 63.73 ± 0.22 & {[}{]} ± {[}{]} & {[}{]} ± {[}{]} & 61.66 ± 0.17 & 59.10 ± 0.14 & 63.63 ± 0.19 
\end{tabular}
\caption{Accuracy}
\label{table:noise15and40}
\end{table}
